Counter Turing Test CT^2: AI-Generated Text Detection is Not as Easy as You May Think -- Introducing AI Detectability Index

With the rise of prolific ChatGPT, the risk and consequences of AI-generated text has increased alarmingly. To address the inevitable question of ownership attribution for AI-generated artifacts, the US Copyright Office released a statement stating that 'If a work's traditional elements of authorship were produced by a machine, the work lacks human authorship and the Office will not register it'. Furthermore, both the US and the EU governments have recently drafted their initial proposals regarding the regulatory framework for AI. Given this cynosural spotlight on generative AI, AI-generated text detection (AGTD) has emerged as a topic that has already received immediate attention in research, with some initial methods having been proposed, soon followed by emergence of techniques to bypass detection. This paper introduces the Counter Turing Test (CT^2), a benchmark consisting of techniques aiming to offer a comprehensive evaluation of the robustness of existing AGTD techniques. Our empirical findings unequivocally highlight the fragility of the proposed AGTD methods under scrutiny. Amidst the extensive deliberations on policy-making for regulating AI development, it is of utmost importance to assess the detectability of content generated by LLMs. Thus, to establish a quantifiable spectrum facilitating the evaluation and ranking of LLMs according to their detectability levels, we propose the AI Detectability Index (ADI). We conduct a thorough examination of 15 contemporary LLMs, empirically demonstrating that larger LLMs tend to have a higher ADI, indicating they are less detectable compared to smaller LLMs. We firmly believe that ADI holds significant value as a tool for the wider NLP community, with the potential to serve as a rubric in AI-related policy-making.

==> author.tex <==
% Megha Chakraborty, S.M Towhidul Islam Tonmoy, S M Mehedi Zaman, Krish Sharma, Niyar R Barman,\\ Chandan Gupta, Shreya Gautam, Tanay Kumar, Vinija Jain, Aman Chadha, Amit P. Sheth, Amitava Das \\


==> img/srl_example.tex <==
\tiny
{
\begin{tabular}{|ll|}
\hline Claim. & \textcolor{red}{Moderna’s lawsuits against Pfizer-BioNTech}
\\ & \textcolor{red}{show COVID-19 vaccines were in} \\
& \textcolor{red}{the works before the pandemic started.} \\
\textcolor{blue}{Verbs.} & [    were, started] \\
\textcolor{blue}{Who.} & [(ARG0 : None, None)] \\
\textcolor{blue}{What.} & [(ARG1 : COVID-19 vaccines, the pandemic)] \\
\textcolor{blue}{Why.} & [(ARGM-TMP : None, None)] \\
\textcolor{blue}{When.} & [(ARGM-LOC : before the pandemic started, None) ] \\
\textcolor{blue}{Why.} & [(ARGM-TMP : None, None)] \\
\textcolor{blue}{Where.} & [(ARGM-CAU : None, None)] \\
\hline
\end{tabular}
}


==> img/srl_example_2.tex <==
\tiny
{
\begin{tabular}{|ll|}
\hline Claim. &  \textcolor{red}{Kamala Harris said that the new and proposed \\ & \textcolor{red}{state laws on voting mean 'if you are going} \\ & \textcolor{red}{to be standing in that line for all those hours, \\ & \textcolor{red}{you can’t have any food.'}} \\
 \textcolor{blue}{Verbs.} & [said, proposed,voting,are,going,be,standing,can't,have] \\
 \textcolor{blue}{Who.} & [(ARG0 : Kamala Harris, None, None, None, None,\\ & None, None, None, you)] \\
 \textcolor{blue}{What.} & [(ARG1 : that the new and proposed state laws on \\ & voting mean 'if you are going to be standing in that\\ &  line for all those hours',you ca n't have any food, state\\ & laws, None, None,\\ & None, None, you, None, any food)] \\
 \textcolor{blue}{Why.} & [(ARGM-TMP : None, None, None, None, None, None,\\ & None, None, None)] \\
 \textcolor{blue}{When.} & [(ARGM-LOC : None, None, None, None, None,\\ & None, for all those hours, None, None)] \\
 \textcolor{blue}{Where.} & [(ARGM-CAU : None, None, None, None, None,\\ & None, None, None, None)] \\
\hline
\end{tabular}
}

==> nlc_figure.tex <==
% \begin{comment}

\begin{figure}[hb!]
\vspace{-2mm}
    \centering
    \includegraphics[width=0.95\columnwidth, height=2cm]{img/opt-nlc.png}
    \vspace{-3mm}
    \caption{NLC comparison for human and OPT-generated text.}
    \label{fig:OPT_NLL}
\vspace{-3mm}
\end{figure}
% \end{comment}

==> scratch.tex <==
\begin{comment}
\begin{table*}[!h]
% \setlength\extrarowheight{2pt}
\centering
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{clll}
\hline
\textbf{GPT-2} & \includegraphics[width=\columnwidth]{img/gpt-perp-histplot.png} & \includegraphics[width=\columnwidth]{img/gpt-perp-lineplot.png}\\ 
\\\hline\\ 
\textbf{OPT} & \includegraphics[width=\columnwidth]{img/opt-perp-histplot.png} & \includegraphics[width=\columnwidth]{img/opt-perp-lineplot.png}\\ 
\\\hline\\ 
\textbf{BLOOM} & \includegraphics[width=\columnwidth]{img/Bloom-perp-histplot.png} & \includegraphics[width=\columnwidth]{img/Bloom-perp-lineplot.png}\\ 
\\\hline\\ 
\textbf{XLNet} & \includegraphics[width=\columnwidth]{img/xlnet-perp-histplot.png} & \includegraphics[width=\columnwidth]{img/xlnet-perp-lineplot.png}\\ 
\\\hline\\ 
 
 
\end{tabular}%
}
\caption{Comparative Study of Perplexity Graph shows overlapping of AI Texts and Human Texts in models GPT-2, OPT, BLOOM and XLNet} 
\label{table:1} 
\end{table*}    
\end{comment}
 

\begin{comment}
\begin{figure}
  \centering
  \includegraphics[width=0.9\textwidth]{img/confusion_matrix.png}
  \caption{Heatmap of 15 LLMs}
  \label{fig:HeatMap}
\end{figure}    
\end{comment}

\begin{comment}
\begin{table*}[!ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ | p{0.06\textwidth} |
                   p{0.55\textwidth} |
                   p{0.02\textwidth} |
                   p{0.02\textwidth} |
                   p{0.55\textwidth} |
                   p{0.02\textwidth} |
                   p{0.02\textwidth} |}
\toprule
 &
   &
  \textbf{\rotatebox[origin=c]{90}{Z-score}} &
  \textbf{\rotatebox[origin=c]{90}{p-value}} &
   &
 \textbf{\rotatebox[origin=c]{90}{Z-score}} &
 \textbf{\rotatebox[origin=c]{90}{p-value}} \\ \midrule
\textbf{Prompt} &
  \textit{Will the next great writer be a robot?} &
   &
   &
 \textit{Detecting AI-generated text is challenging but not impossible. Ongoing efforts improve accuracy and uphold transparency.} &
   &
   \\ \hline
\textbf{\rotatebox[origin=r]{90}{\parbox[c]{2cm}{\centering Watermarked text}}}
    &
    {I'm \colorbox{pink}{very skeptical} that the next "great writer" is going to be a robot, \colorbox{pink}{or} that they'll be \colorbox{pink}{much} more effective at \colorbox{pink}{expressing the} subtleties and depths of \colorbox{pink}{human} thought than a human is. However, what is \colorbox{pink}{most} interesting is the role that the \colorbox{pink}{Internet could} play in bringing these "robot" writers into the public eye. If I could (and I'm \colorbox{pink}{very} excited by this possibility), I would pay a \colorbox{pink}{small monthly} fee to \colorbox{pink}{read well-written}...}
   & \rotatebox[origin=c]{90}{\parbox[r]{1.5cm}{\centering 4.24}}
   & \rotatebox[origin=c]{90}{\parbox[r]{2cm}{\centering 1.1e-05}}
   &
   AI has made \colorbox{pink}{great} strides, and the potential of these technologies to \colorbox{pink}{improve} our lives is enormous. However, AI \colorbox{pink}{also} can pose ethical and \colorbox{pink}{social} challenges.
In this article, we discuss some of the ways AI text analysis is used to generate \colorbox{pink}{harmful language}, and the \colorbox{pink}{work} being undertaken to detect and prevent it. We also discuss some \colorbox{pink}{recent work} aimed at \colorbox{pink}{ensuring transparency} and interoperability in text analysis. 
& \rotatebox[origin=c]{90}{\parbox[r]{1.5cm}{\centering 5.06}}
   & \rotatebox[origin=c]{90}{\parbox[r]{1.5cm}{\centering 2.06e-07}}
   \\ \hline
\textbf{\rotatebox[origin=r]{90}{\parbox[c]{5cm}{\centering De-Watermarked text by replacing high-entropy words}}} &
    {I'm \colorbox{green}{somewhat} skeptical that the next "great writer" is going to be a robot, \colorbox{green}{given} that they'll be \colorbox{green}{far} more effective at \colorbox{green}{grasping deeper} subtleties and depths of philosophical thought than a robot is. However, what is \colorbox{green}{particularly} interesting is the role that the Internet \colorbox{green}{may} play in bringing new great writers into the public eye. If I did (and I'm \colorbox{green}{extremely} excited by this possibility), I would pay a \colorbox{green}{hefty subscription} fee to \colorbox{green}{publish  something}}...
   & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 1.76 \textcolor{red}{[58.5\% \Downarrow}]}}
   &     \rotatebox[origin=c]{90}{\parbox[r]{4cm}{\centering 0.039\textcolor{red}{[3.5e05\% \Uparrow}]}}
   &
   AI has made \colorbox{green}{tremendous} strides and the potential of these technologies to \colorbox{green}{transform} our lives is exciting However, AI \colorbox{green}{manipulation} can pose ethical and \colorbox{green}{legal} challenges. In this article, we discuss some of the ways AI text analysis is used to generate \colorbox{green}{artificial speech} and the \colorbox{green}{measures} being undertaken to detect and prevent it. We also discuss some \colorbox{green}{important steps} aimed at \colorbox{green}{improving accuracy} and interoperability in text analysis. & 
    \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 3.72 \textcolor{red}{[26.48\% \Downarrow}]}}
    
   &     \rotatebox[origin=c]{90}{\parbox[r]{4cm}{\centering 9.96e-05 \textcolor{red}{[4.8e04\% \Uparrow}]}}
   \\ \hline
\textbf{\rotatebox[origin=r]{90}{\parbox[c]{5cm}{\centering De-Watermarked text by paraphrasing}}} &
    I have \colorbox{cyan}{serious doubts} about the possibility of a robot becoming the next \colorbox{cyan}{exceptional writer} and \colorbox{cyan}{surpassing humans} in expressing the nuances and profoundness of human thoughts. Nevertheless, what \colorbox{cyan}{fascinates} me the most is the potential impact of the \colorbox{cyan}{Internet in showcasing} these "robot" writers to the general public. The idea of being able to pay a \colorbox{cyan}{nominal monthly} subscription fee to access \colorbox{cyan}{impeccably written} and carefully refined works \colorbox{cyan}{truly} thrills me...
   & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering -0.542 \textcolor{red}{[112.78\% \Downarrow}]}}
   & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 0.706 \textcolor{red}{[6.4e6\% \Uparrow}]}}

   &
The \colorbox{cyan}{advancements} in AI have been significant and hold immense potential for \colorbox{cyan}{enhancing} our daily lives. Nevertheless, there are ethical and \colorbox{cyan}{societal} \colorbox{cyan}{concerns} that come with the use of AI. This piece delves into the \colorbox{cyan}{negative impact} of AI-generated language and the \colorbox{cyan}{measures being taken} to identify and prevent it. Additionally, we explore \colorbox{cyan}{recent efforts} to \colorbox{cyan}{promote transparency} and compatibility in text analysis.  & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 0.593 \textcolor{red}{[88.28\% \Downarrow}]}}
   & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 0.276 \textcolor{red}{[1.3e8\% \Uparrow}]}}

   \\ \bottomrule
\end{tabular}%
}
\end{table*}
\end{comment}

\begin{comment}
\begin{table*}[!ht]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{ 
                p{0.15\textwidth} |
                p{0.65\textwidth}  |
                P{0.1\textwidth} |
                P{0.1\textwidth}
}
\toprule
 &
   &
  \textbf{{{\scriptsize Z-score}}} &
  \textbf{{{\scriptsize p-value}}}
  \\ \toprule
\textbf{{\scriptsize Prompt}} &
  \textit{{\scriptsize Will the next great writer be a robot?}} &
   &
   \\ \hline
%\textbf{\rotatebox[origin=r]{90}{\parbox[r]{1cm}{\centering {\footnotesize Watermarked text}}}}
\textbf{{\scriptsize Watermarked text}}
    &
    {
    \begin{scriptsize}
    I'm \colorbox{pink}{very skeptical} that the next "great writer" is going to be a robot, \colorbox{pink}{or} that they'll be \colorbox{pink}{much} more effective at \colorbox{pink}{expressing the} subtleties and depths of \colorbox{pink}{human} thought than a human is. However, what is \colorbox{pink}{most} interesting is the role that the \colorbox{pink}{Internet could} play in bringing these "robot" writers into the public eye. If I could (and I'm \colorbox{pink}{very} excited by this possibility), I would pay a \colorbox{pink}{small monthly} fee to \colorbox{pink}{read well-written}...
    \end{scriptsize}
    }
   & \scriptsize 4.24
   % {\parbox[r]{1cm}{\centering }}
   & \scriptsize $1.1\times10^{-5}$
   % {\parbox[r]{1cm}{\centering 1.1e-05}}
   \\ \hline
%\textbf{\rotatebox[origin=r]{90}{\parbox[c]{1cm}{\centering {\footnotesize De-Watermarked text by replacing high-entropy words}}}} &
\textbf{{\scriptsize De-Watermarked text by replacing high-entropy words}} &
    {
    \begin{scriptsize}
    I'm \colorbox{green}{somewhat} skeptical that the next "great writer" is going to be a robot, \colorbox{green}{given} that they'll be \colorbox{green}{far} more effective at \colorbox{green}{grasping deeper} subtleties and depths of philosophical thought than a robot is. However, what is \colorbox{green}{particularly} interesting is the role that the Internet \colorbox{green}{may} play in bringing new great writers into the public eye. If I did (and I'm \colorbox{green}{extremely} excited by this possibility), I would pay a \colorbox{green}{hefty subscription} fee to \colorbox{green}{publish  something}...
    \end{scriptsize}
    }
   & \scriptsize 1.76 \newline \textcolor{red}{(58.5\%} \color{red} \Downarrow)
   % {\parbox[r]{1cm}{\centering 1.76 \textcolor{red}{[58.5\% \Downarrow}]}}
   & \scriptsize 0.039 \newline \textcolor{red}{($3.5\times10^5$\%} \color{red} \Uparrow)
   % {\parbox[r]{1cm}{\centering 0.039 \textcolor{red}{[3.5e05\% \Uparrow}]}}
   
   \\ \hline
%\textbf{\rotatebox[origin=r]{90}{\parbox[c]{1cm}{\centering {\footnotesize De-Watermarked text by paraphrasing}}}} &
\textbf{{\scriptsize De-Watermarked text by paraphrasing}} &
    \begin{scriptsize}
    I have \colorbox{cyan}{serious doubts} about the possibility of a robot becoming the next \colorbox{cyan}{exceptional writer} and \colorbox{cyan}{surpassing humans} in expressing the nuances and profoundness of human thoughts. Nevertheless, what \colorbox{cyan}{fascinates} me the most is the potential impact of the \colorbox{cyan}{Internet in showcasing} these "robot" writers to the general public. The idea of being able to pay a \colorbox{cyan}{nominal monthly} subscription fee to access \colorbox{cyan}{impeccably written} and carefully refined works \colorbox{cyan}{truly} thrills me...
    \end{scriptsize}
   & \scriptsize -0.542 \newline \textcolor{red}{(112.8\%} \color{red} \Downarrow)
   % {\parbox[b]{1cm}{\centering -0.542 \textcolor{red}{[112.78\% \Downarrow}]}}
   & \scriptsize 0.706 \newline \textcolor{red}{($6.4\times10^6$\%} \color{red} \Uparrow)
   % {\parbox[b]{1cm}{\centering 0.706 \textcolor{red}{[6.4e6\% \Uparrow}]}}

   \\ \bottomrule
\end{tabular}%
}
\caption{An illustration of de-watermarking by replacing high-entropy words and paraphrasing. DetectGPT classifies a text to be
generated by GPT-2 if the z-score is greater than 4.}
\label{tab:dewatermarking_table_2}
\end{table*}   
\end{comment}

\begin{comment}
\begin{table*}[!h]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{ 
                p{0.15\textwidth} |
                p{0.65\textwidth}  |
                P{0.1\textwidth} |
                P{0.1\textwidth}
}
\toprule
 &
   &
  \textbf{{{\scriptsize Z-score}}} &
  \textbf{{{\scriptsize p-value}}}
  \\ \toprule
\textbf{{\scriptsize Prompt}} &
  \textit{{\scriptsize Will the next great writer be a robot?}} &
   &
   \\ \hline
%\textbf{\rotatebox[origin=r]{90}{\parbox[r]{1cm}{\centering {\footnotesize Watermarked text}}}}
\textbf{{\scriptsize Watermarked text}}
    &
    {
    \begin{scriptsize}
    I'm \colorbox{pink}{very skeptical} that the next "great writer" is going to be a robot, \colorbox{pink}{or} that they'll be \colorbox{pink}{much} more effective at \colorbox{pink}{expressing the} subtleties and depths of \colorbox{pink}{human} thought than a human is. However, what is \colorbox{pink}{most} interesting is the role that the \colorbox{pink}{Internet could} play in bringing these "robot" writers into the public eye. If I could (and I'm \colorbox{pink}{very} excited by this possibility), I would pay a \colorbox{pink}{small monthly} fee to \colorbox{pink}{read well-written}...
    \end{scriptsize}
    }
   & \scriptsize 4.24
   % {\parbox[r]{1cm}{\centering }}
   & \scriptsize $1.1\times10^{-5}$
   % {\parbox[r]{1cm}{\centering 1.1e-05}}
   \\ \hline
%\textbf{\rotatebox[origin=r]{90}{\parbox[c]{1cm}{\centering {\footnotesize De-Watermarked text by replacing high-entropy words}}}} &
\textbf{{\scriptsize De-Watermarked text by replacing high-entropy words}} &
    {
    \begin{scriptsize}
    I'm \colorbox{green}{somewhat} skeptical that the next "great writer" is going to be a robot, \colorbox{green}{given} that they'll be \colorbox{green}{far} more effective at \colorbox{green}{grasping deeper} subtleties and depths of philosophical thought than a robot is. However, what is \colorbox{green}{particularly} interesting is the role that the Internet \colorbox{green}{may} play in bringing new great writers into the public eye. If I did (and I'm \colorbox{green}{extremely} excited by this possibility), I would pay a \colorbox{green}{hefty subscription} fee to \colorbox{green}{publish  something}...
    \end{scriptsize}
    }
   & \scriptsize 1.76 \newline \textcolor{red}{(58.5\%} \color{red} \Downarrow)
   % {\parbox[r]{1cm}{\centering 1.76 \textcolor{red}{[58.5\% \Downarrow}]}}
   & \scriptsize 0.039 \newline \textcolor{red}{($3.5\times10^5$\%} \color{red} \Uparrow)
   % {\parbox[r]{1cm}{\centering 0.039 \textcolor{red}{[3.5e05\% \Uparrow}]}}
   
   \\ \hline
%\textbf{\rotatebox[origin=r]{90}{\parbox[c]{1cm}{\centering {\footnotesize De-Watermarked text by paraphrasing}}}} &
\textbf{{\scriptsize De-Watermarked text by paraphrasing}} &
    \begin{scriptsize}
    I have \colorbox{cyan}{serious doubts} about the possibility of a robot becoming the next \colorbox{cyan}{exceptional writer} and \colorbox{cyan}{surpassing humans} in expressing the nuances and profoundness of human thoughts. Nevertheless, what \colorbox{cyan}{fascinates} me the most is the potential impact of the \colorbox{cyan}{Internet in showcasing} these "robot" writers to the general public. The idea of being able to pay a \colorbox{cyan}{nominal monthly} subscription fee to access \colorbox{cyan}{impeccably written} and carefully refined works \colorbox{cyan}{truly} thrills me...
    \end{scriptsize}
   & \scriptsize -0.542 \newline \textcolor{red}{(112.8\%} \color{red} \Downarrow)
   % {\parbox[b]{1cm}{\centering -0.542 \textcolor{red}{[112.78\% \Downarrow}]}}
   & \scriptsize 0.706 \newline \textcolor{red}{($6.4\times10^6$\%} \color{red} \Uparrow)
   % {\parbox[b]{1cm}{\centering 0.706 \textcolor{red}{[6.4e6\% \Uparrow}]}}

   \\ \bottomrule
\end{tabular}%
}
\caption{An illustration of de-watermarking by replacing high-entropy words and paraphrasing. DetectGPT classifies a text to be
generated by GPT-2 if the z-score is greater than 4.}
\label{tab:dewatermarking_table_3}
\end{table*}    
\end{comment}


% ------------------------------------------------
dewatermarking after paraphrasing for all llms
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \begin{table}[h!]


% \begin{table}[!htbp]
% \centering
% \resizebox{0.65\columnwidth}{!}{%
% \begin{tabular}{ccccccc}
% \hline
% \multirow{3}{*}{Models} & \multicolumn{6}{c}{Paraphrase}                                                      \\ \cline{2-7} 
%                         & \multicolumn{2}{c}{GPT-3} & \multicolumn{2}{c}{Pegasus} & \multicolumn{2}{c}{T5}    \\ \cline{2-7} 
%                         & v1             & v2       & v1              & v2        & v1                   & v2 \\ \hline
% OPT                     & 100.0\%        &          & 100.0\%         &           & \multicolumn{1}{l}{} &    \\
% Alpaca                  & 95.0\%         &          & 95.5\%          &           & \multicolumn{1}{l}{} &    \\
% T0                      & 98.0\%         &          & 96.8\%          &           & 83.9\%               &    \\
% MPT7B                   & 96.0\%         &          & 88.5\%          &           &                      &    \\
% Vicuna                  & 98.0\%         &          & 98.7\%          &           &                      &    \\
% FlanT5                  & 100.0\%        &          & 99.0\%          &           &                      &    \\
% Dolly                   & 98.0\%         &          & 95.6\%          &           &                      &    \\
% StableLM                & 95.0\%         &          & 100.0\%         &           & 83.0\%               &    \\
% LLAMA                   & 95.0\%         &          & 89.3\%          &           &                      &    \\
% BLOOM                   & 97.0\%         &          & 87.2\%          &           &                      &    \\
% XLNET                   & 100.0\%        &          & 100.0\%         &           & 63.3\%               &   \\
% \bottomrule
% \end{tabular}
% }
% \caption{dewatermarking after paraphrasing for all llms}
% \label{tab:para-dewm-all}
% \end{table}


% ------------------------------------------------

% ------------------------------------------------
\begin{comment}
\begin{longtblr}[
  caption = {Text Perturbations and NLC Values Analysis},
  label = {tab:example1},
]{
  colspec = {|X|X[4]|X[1]|},
  rowhead = 1,
  hlines,
} 
\textbf{{\footnotesize Input Type}}  &  \textbf{{\footnotesize Input}} & \textbf{{\footnotesize NLC Value}} \\
\textbf{{\footnotesize GPT 4 Generated Text}}  &     \begin{footnotesize}
Treasury Secretary Janet Yellen made history in December by becoming the first woman to put her signature on U.S. bank notes. It also marked one of the rare occasions when the nation's currency has been remade. In the case of the 2017 \$10 Bill, the security for this \$100 Bill (the date on top of the new \$100 Bill) is actually embedded in the \$20 Bill. A new security thread is pulled out, thread which is pulled into the \$10 Bill to form a loop that allows for easier manufacture. The change in date is something that comes up every few years. The date on a \$100 Bill was determined by the Congress of the United States. They changed it several times during the 19th century. Then in 1942, the Congress moved towards date accuracy and made an amendment to the U.S. Constitution stating that the date printed on public money will be the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.456} \\
\textbf{{\footnotesize GPT 4 Text Perturbations}}  &     \begin{footnotesize}
    In December, Treasury Secretary Janet Yellen etched her name into history as the first woman to sign U.S. bank notes, bringing about a rare transformation of the nation's currency. The 2017 \$10 Bill has a unique security feature tied to the \$100 Bill: a concealed thread from the \$20 Bill is carefully extracted and threaded into the \$10 Bill, creating a loop that streamlines the manufacturing process. Adjusting the date on banknotes is a periodic occurrence, and the Congress of the United States has altered the date on the \$100 Bill multiple times throughout the 19th century. However, in 1942, an amendment to the U.S. Constitution mandated that the date printed on public money must reflect the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.491} \\
\textbf{{\footnotesize }}  &     \begin{footnotesize}
    Making history in December, Treasury Secretary Janet Yellen became the first woman to leave her mark on U.S. bank notes, initiating a rare transformation of the nation's currency. The 2017 \$10 Bill introduces a fascinating security measure tied to the \$100 Bill: an embedded thread from the \$20 Bill is carefully unraveled and integrated into the \$10 Bill, forming a practical loop that enhances the manufacturing process. Modifying the date on banknotes arises periodically, and over the course of the 19th century, the Congress of the United States made several adjustments to the date on the \$100 Bill. However, in 1942, the Congress took a step towards precision by amending the U.S. Constitution to mandate that the date imprinted on public money must represent the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.405} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
    December marked a significant moment as Treasury Secretary Janet Yellen etched her name into the annals of history as the first woman to autograph U.S. bank notes, initiating a rare redesign of the nation's currency. The 2017 \$10 Bill incorporates a unique security feature associated with the \$100 Bill: a concealed thread, originally part of the \$20 Bill, is meticulously withdrawn and integrated into the \$10 Bill, forming a convenient loop that streamlines the manufacturing process. Altering the date on banknotes is a recurring event, and throughout the 19th century, the Congress of the United States made several modifications to the date on the \$100 Bill. However, in 1942, the Congress emphasized accuracy by amending the U.S. Constitution to stipulate that the date printed on public money must reflect the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.421} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
    In a historic move, Treasury Secretary Janet Yellen made her mark in December as the first woman to sign U.S. bank notes, triggering a rare overhaul of the nation's currency. The 2017 \$10 Bill incorporates a distinctive security element linked to the \$100 Bill: a hidden thread from the \$20 Bill is carefully extracted and incorporated into the \$10 Bill, creating a practical loop that facilitates the manufacturing process. Adjusting the date on banknotes is a periodic occurrence, and during the 19th century, the Congress of the United States made several changes to the date on the \$100 Bill. However, in 1942, the Congress sought precision by amending the U.S. Constitution to mandate that the date imprinted on public money must represent the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.507} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
    December witnessed a momentous occasion as Treasury Secretary Janet Yellen etched her name into the history books, becoming the first woman to sign U.S. bank notes and instigating a rare transformation of the nation's currency. The 2017 \$10 Bill incorporates an intriguing security feature tied to the \$100 Bill: a concealed thread, originally belonging to the \$20 Bill, is meticulously pulled out and integrated into the \$10 Bill, forming a practical loop that streamlines the manufacturing process. Modifying the date on banknotes is a recurring event, and throughout the 19th century, the Congress of the United States made multiple adjustments to the date on the \$100 Bill. However, in 1942, the Congress embraced accuracy by amending the U.S. Constitution to specify that the date printed on public money must represent the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.535} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
    Making history in December, Treasury Secretary Janet Yellen became the first woman to grace U.S. bank notes with her signature, ushering in a rare transformation of the nation's currency. The 2017 \$10 Bill introduces a unique security element tied to the \$100 Bill: a concealed thread extracted from the \$20 Bill is skillfully woven into the \$10 Bill, creating a loop that streamlines the manufacturing process. Adjusting the date on banknotes is a periodic occurrence, and throughout the 19th century, the Congress of the United States modified the date on the \$100 Bill on several occasions. However, in 1942, the Congress pursued accuracy by amending the U.S. Constitution, mandating that the date imprinted on public money must reflect the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.518} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
December marked a historic milestone as Treasury Secretary Janet Yellen became the first woman to leave her signature on U.S. bank notes, instigating a rare overhaul of the nation's currency. The 2017 \$10 Bill features a distinctive security mechanism connected to the \$100 Bill: an embedded thread, originally part of the \$20 Bill, is carefully extracted and incorporated into the \$10 Bill, forming a loop that simplifies the manufacturing process. Modifying the date on banknotes is a recurring event, and throughout the 19th century, the Congress of the United States made several changes to the date on the \$100 Bill. However, in 1942, the Congress prioritized accuracy by amending the U.S. Constitution to require that the date printed on public money must represent the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.556} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
In a momentous event, Treasury Secretary Janet Yellen etched her name into the annals of history in December by becoming the first woman to inscribe U.S. bank notes, heralding a rare transformation of the nation's currency. The 2017 \$10 Bill incorporates a unique security feature tied to the \$100 Bill: a concealed thread from the \$20 Bill is meticulously extracted and woven into the \$10 Bill, forming a loop that facilitates easier manufacturing. Changing the date on banknotes is a recurring process, and throughout the 19th century, the Congress of the United States made several alterations to the date on the \$100 Bill. However, in 1942, the Congress moved towards accuracy by amending the U.S. Constitution to specify that the date printed on public money must correspond to the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.423} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
December witnessed a groundbreaking moment as Treasury Secretary Janet Yellen left her indelible mark on U.S. bank notes, becoming the first woman to do so and prompting a rare remaking of the nation's currency. The 2017 \$10 Bill introduces an intriguing security feature associated with the \$100 Bill: a concealed thread from the \$20 Bill is carefully pulled out and integrated into the \$10 Bill, creating a loop that streamlines the manufacturing process. Modifying the date on banknotes is a recurring occurrence, and throughout the 19th century, the Congress of the United States made several changes to the date on the \$100 Bill. However, in 1942, the Congress pursued date accuracy by amending the U.S. Constitution to mandate that the date printed on public money must represent the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.424} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
Treasury Secretary Janet Yellen etched her name into history in December, breaking barriers as the first woman to leave her signature on U.S. bank notes and catalyzing a rare transformation of the nation's currency. The 2017 \$10 Bill incorporates a unique security feature connected to the \$100 Bill: a concealed thread from the \$20 Bill is meticulously extracted and incorporated into the \$10 Bill, forming a loop that simplifies the manufacturing process. Adjusting the date on banknotes is a periodic event, and throughout the 19th century, the Congress of the United States made multiple modifications to the date on the \$100 Bill. However, in 1942, the Congress took a step towards precision by amending the U.S. Constitution to stipulate that the date printed on public money must reflect the original year of the United States.
    \end{footnotesize} & {\footnotesize 1.472} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
Treasury Secretary Janet Yellen made history in December when she became the first woman to sign US bank notes. It was also one of the few times when the country's currency was rebuilt. The security for this \$100 Bill (the date on top of the new \$100 Bill) is actually integrated in the 2017 \$10 Bill. A new security thread is extracted, which is then inserted into the \$10 bill to make a loop that allows for simpler manufacturing. The date change is something that happens every few years. The date on a \$100 bill was set by the United States Congress. 
    \end{footnotesize} & {\footnotesize 1.497} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
Treasury Secretary Janet Yellen carved her name into history in December, becoming the first woman to sign U.S. bank notes and sparking a remarkable makeover of the country's currency. The 2017 \$10 bill has a one-of-a-kind security feature linked to the \$100 bill: a hidden thread from the \$20 bill is methodically retrieved and inserted into the \$10 bill, producing a loop that streamlines the manufacturing process. Changing the date on banknotes is a regular occurrence, and the Congress of the United States made many changes to the date on the \$100 bill throughout the nineteenth century. However, in 1942, Congress took a step towards precision by amending the United States Constitution to require that the date printed on public documents be precise.
    \end{footnotesize} & {\footnotesize 1.582} \\
\textbf{{\footnotesize }}  &     \begin{footnotesize}
Treasury Secretary Janet Yellen made history in December by becoming the first woman to inscribe U.S. bank notes, ushering in a unique makeover of the nation's currency. The 2017 \$10 bill includes a novel security element that is linked to the \$100 bill: a secret thread from the \$20 bill is precisely retrieved and weaved into the \$10 bill, making a loop that allows for easier manufacture. Changing the date on banknotes is a common practise, and the Congress of the United States made multiple changes to the date on the \$100 bill over the nineteenth century. However, in 1942, Congress took a step towards accuracy by amending the United States Constitution to require that the date written on public money be accurate. 
    \end{footnotesize} & {\footnotesize 1.483} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
Treasury Secretary Janet Yellen made history in December when she became the first woman to signature U.S. bank notes, kicking off an unusual overhaul of the country's currency. The 2017 \$10 bill has a novel security element similar to the \$100 bill: a secret thread, previously part of the \$20 bill, is precisely extracted and merged into the \$10 bill, making a handy loop that speeds the production process. Changing the date on banknotes is a common occurrence, and the Congress of the United States made multiple changes to the date on the \$100 bill over the nineteenth century. However, by modifying the United States Code in 1942, Congress emphasised accuracy.  
    \end{footnotesize} & {\footnotesize 1.434} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
In an unusual change to the nation's currency in December, Treasury Secretary Janet Yellen became the first woman to put her signature on a U.S. bank note. An intriguing security feature associated with the 2017 \$10 bill is introduced: a thread from the \$20 bill is meticulously untangled and inserted into the \$10 bill, creating a useful loop that improves the manufacturing process. Periodically, the need to change the date on banknotes arises, and throughout the 19th century, the United States Congress changed the date on the \$100 bill multiple times. 
    \end{footnotesize} & {\footnotesize 1.499} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
As the first woman to stamp her name on American banknotes, Treasury Secretary Janet Yellen made history in December by launching a rare reform of the country's currency. The 2017 \$10 bill has a unique security element that is linked to the 2017 \$100 bill: an embedded thread that was once a component of the 2017 \$20 bill is carefully removed and inserted into the 2017 \$10 bill, creating a loop that makes the manufacturing process easier. The date on banknotes is frequently changed, and the United States Congress changed the date on the \$100 bill multiple times over the 19th century.  
    \end{footnotesize} & {\footnotesize 1.512} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
When Treasury Secretary Janet Yellen became the first woman to do so on American bank notes in December, it was a historic milestone that led to a rare reprint of the country's money. A clever security feature linked with the 2017 \$10 bill is introduced: a hidden thread from the 2017 \$20 bill is carefully plucked out and inserted into the 2017 \$10 bill, streamlining the production process. This security element was previously only found on the 2017 \$100 bill. The date on banknotes is frequently changed, and the United States Congress changed the date on the \$100 bill multiple times over the 19th century.   
    \end{footnotesize} & {\footnotesize 1.445} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
As the first woman to sign American bank notes, Treasury Secretary Janet Yellen made history in December and helped transform the nation's currency. The 2017 \$10 note contains a unique security feature connected to the \$100 bill: a thread buried on the \$20 bill is carefully removed and put into the \$10 bill, creating a loop that speeds up production. The United States Congress often altered the date on the \$100 bill throughout the nineteenth century. Date alterations on banknotes are a common occurrence. However, in 1942, Congress made a step towards accuracy by adding a clause to the US Constitution requiring the accuracy of the date stated on official papers.  
    \end{footnotesize} & {\footnotesize 1.464} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
In December, Treasury Secretary Janet Yellen made history by becoming the first woman to have her signature placed on U.S. bank notes, marking the beginning of a rare change to the country's currency. The 2017 \$10 bill adds a special security feature that is linked to the \$100 bill: a hidden thread that was taken from the \$20 bill is expertly weaved into the \$10 bill to create a loop that speeds up production. The date on banknotes is occasionally changed, and the United States Congress changed the date on the \$100 bill multiple times over the 19th century. However, the Congress sought accuracy by amending the U.S. Constitution in 1942, requiring that the date written on government money reflect the year the United States was founded.
    \end{footnotesize} & {\footnotesize 1.456} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
In the month of December, Treasury Secretary Janet Yellen became the first woman to sign US bank notes, ushering in a unique makeover of the nation's currency. The 2017 \$10 Bill contains a new security feature that is linked to the \$100 Bill: a hidden thread removed from the \$20 Bill is carefully weaved into the \$10 Bill, forming a loop that speeds the production process. The date on banknotes is adjusted on a regular basis, and the Congress of the United States changed the date on the \$100 bill multiple times throughout the nineteenth century. However, in 1942, Congress sought accuracy by modifying the United States Constitution to require that the year engraved on public money match the country's founding year.  
    \end{footnotesize} & {\footnotesize 1.423} \\
\textbf{{\footnotesize Human Written Text}}  &    \begin{footnotesize}
    Cash may seem old-fashioned these days. Especially as debates over digital currencies make headlines and Treasury Secretary Janet L. Yellen is fielding questions about ideas to mint a trillion-dollar platinum coin to avert a debt ceiling crisis. But in much of the world, cash is still king. In December, Ms. Yellen made history during a trip to the Bureau of Engraving and Printing in Fort Worth, Texas, where she signed commemorative notes at the unveiling of a new batch of dollar bills.
    \end{footnotesize} & {\footnotesize 1.551} \\
\textbf{{\footnotesize Human Text Perturbations}}  &     \begin{footnotesize}
    Cash may appear outdated in today's world, particularly with the rise of digital currencies and discussions surrounding the creation of a trillion-dollar platinum coin to address the debt ceiling issue, a topic Treasury Secretary Janet L. Yellen is actively addressing. However, in many parts of the globe, cash remains the preferred form of payment. During her visit to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Ms. Yellen left her mark by signing commemorative notes at the unveiling of a fresh set of dollar bills.
    \end{footnotesize} & {\footnotesize 1.481} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
   As digital currencies dominate the headlines and the idea of minting a trillion-dollar platinum coin to tackle the debt ceiling crisis gains attention, the value of cash may seem antiquated. Nevertheless, cash continues to reign supreme in various parts of the world. In a notable event at the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen etched her name on commemorative notes during the introduction of a new series of dollar bills.
    \end{footnotesize} & {\footnotesize 1.504} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
   In the face of ongoing debates about digital currencies and proposals like the creation of a trillion-dollar platinum coin to manage the debt ceiling, cash can appear to belong to a bygone era. However, in many regions worldwide, cash remains the preferred medium of exchange. In a historic occasion at the Bureau of Engraving and Printing in Fort Worth, Texas, back in December, Treasury Secretary Janet L. Yellen left her mark by signing commemorative notes when unveiling a fresh batch of dollar bills.
    \end{footnotesize} & {\footnotesize 1.516} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
   With the spotlight on digital currencies and discussions surrounding the minting of a trillion-dollar platinum coin to address the debt ceiling crisis, the relevance of cash may seem diminished in today's world. Yet, cash still holds its status as king in many parts of the globe. In a momentous event during her visit to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen made history by autographing commemorative notes at the unveiling of a new collection of dollar bills.
    \end{footnotesize} & {\footnotesize 1.486} \\
     \textbf{{\footnotesize }}  &     \begin{footnotesize}
   The prominence of digital currencies and the proposal of minting a trillion-dollar platinum coin as a solution to the debt ceiling crisis can make cash appear outmoded in contemporary times. Nevertheless, cash retains its dominance in numerous regions worldwide. Notably, in December, Treasury Secretary Janet L. Yellen created a significant moment at the Bureau of Engraving and Printing in Fort Worth, Texas, where she signed commemorative notes during the unveiling of a fresh series of dollar bills.
    \end{footnotesize} & {\footnotesize 1.501} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
   In an era marked by discussions on digital currencies and the concept of minting a trillion-dollar platinum coin to address the debt ceiling crisis, cash may seem like a relic of the past. However, it continues to hold sway as the preferred mode of payment in many parts of the world. In a noteworthy event during her visit to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen made history by signing commemorative notes while introducing a new batch of dollar bills.
    \end{footnotesize} & {\footnotesize 1.518} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
  While the rise of digital currencies and debates surrounding the creation of a trillion-dollar platinum coin to tackle the debt ceiling crisis overshadow the significance of cash, it still reigns supreme in many global economies. Treasury Secretary Janet L. Yellen left a memorable imprint during her trip to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, where she signed commemorative notes at the unveiling of a fresh set of dollar bills.
    \end{footnotesize} & {\footnotesize 1.535} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
 The prevalence of digital currencies and the proposal to mint a trillion-dollar platinum coin to resolve the debt ceiling crisis may give the impression that cash is outdated. However, cash continues to be the preferred medium of exchange in various parts of the world. In a historic moment during her visit to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen left her mark by signing commemorative notes at the unveiling of a new batch of dollar bills.
    \end{footnotesize} & {\footnotesize 1.508} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
 As debates surrounding digital currencies and the idea of minting a trillion-dollar platinum coin to overcome the debt ceiling crisis make headlines, the relevance of cash may appear diminished. Nevertheless, cash remains the reigning champion in many regions worldwide. During a momentous occasion at the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen made history by autographing commemorative notes when unveiling a fresh collection of dollar bills.
    \end{footnotesize} & {\footnotesize 1.551} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
 In an age where digital currencies and the potential creation of a trillion-dollar platinum coin to tackle the debt ceiling issue take center stage, cash may seem like a thing of the past. However, it still holds its status as the primary mode of payment in many parts of the world. During a significant event at the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen left her mark by signing commemorative notes while introducing a new series of dollar bills.
    \end{footnotesize} & {\footnotesize 1.444} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
 With the ongoing discussions revolving around digital currencies and the proposal to mint a trillion-dollar platinum coin to address the debt ceiling crisis, cash might appear outdated. However, it continues to be the preferred mode of payment in various parts of the world. In December, Treasury Secretary Janet L. Yellen made a historic visit to the Bureau of Engraving and Printing in Fort Worth, Texas, where she signed commemorative notes during the unveiling of a new batch of dollar bills.
    \end{footnotesize} & {\footnotesize 1.472} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
 While digital currencies dominate current debates and the concept of minting a trillion-dollar platinum coin captures attention as a solution to the debt ceiling crisis, cash remains the prevailing form of payment in many regions worldwide. In a momentous occasion during her trip to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen left her mark by signing commemorative notes at the unveiling of a fresh collection of dollar bills.
    \end{footnotesize} & {\footnotesize 1.528} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
The increasing prominence of digital currencies and the discussions surrounding the minting of a trillion-dollar platinum coin to alleviate the debt ceiling crisis may lead some to believe that cash is becoming obsolete. However, cash continues to hold its ground as the primary medium of exchange in numerous parts of the world. Treasury Secretary Janet L. Yellen created a historic moment in December when she signed commemorative notes at the Bureau of Engraving and Printing in Fort Worth, Texas, during the introduction of a new series of dollar bills.
    \end{footnotesize} & {\footnotesize 1.466} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
In the midst of debates surrounding digital currencies and the idea of minting a trillion-dollar platinum coin to resolve the debt ceiling crisis, cash may seem like a relic from a bygone era. Nonetheless, it remains the preferred method of payment in many regions across the globe. During her visit to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen etched her name on commemorative notes, marking the unveiling of a fresh batch of dollar bills.
    \end{footnotesize} & {\footnotesize 1.496} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
Amidst the buzz surrounding digital currencies and the proposal to mint a trillion-dollar platinum coin as a solution to the debt ceiling crisis, cash may appear outdated. However, it still holds its status as the dominant mode of payment in various parts of the world. In December, during a significant event at the Bureau of Engraving and Printing in Fort Worth, Texas, Treasury Secretary Janet L. Yellen made history by signing commemorative notes while unveiling a new series of dollar bills.
    \end{footnotesize} & {\footnotesize 1.495} \\
     \textbf{{\footnotesize }}  &     \begin{footnotesize}
With digital currencies taking center stage and discussions revolving around the idea of minting a trillion-dollar platinum coin to tackle the debt ceiling crisis, the significance of cash may seem diminished. However, it remains the reigning king in terms of preferred payment methods in many parts of the world. In a noteworthy event during her visit to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen left her mark by signing commemorative notes at the unveiling of a fresh batch of dollar bills.
    \end{footnotesize} & {\footnotesize 1.473} \\
     \textbf{{\footnotesize }}  &     \begin{footnotesize}
In a world dominated by discussions on digital currencies and the proposal to mint a trillion-dollar platinum coin to address the debt ceiling crisis, cash may seem like a thing of the past. However, it still holds its position as the primary medium of exchange in numerous regions across the globe. In December, during her visit to the Bureau of Engraving and Printing in Fort Worth, Texas, Treasury Secretary Janet L. Yellen made history by signing commemorative notes, marking the unveiling of a new series of dollar bills.
    \end{footnotesize} & {\footnotesize 1.514} \\
     \textbf{{\footnotesize }}  &     \begin{footnotesize}
While debates surrounding digital currencies and the idea of minting a trillion-dollar platinum coin to overcome the debt ceiling crisis grab attention, cash maintains its status as the preferred form of payment in many parts of the world. In a significant event at the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen left a lasting impression by signing commemorative notes during the unveiling of a new collection of dollar bills.
    \end{footnotesize} & {\footnotesize 1.455} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
Despite the prevalence of digital currencies and discussions on the creation of a trillion-dollar platinum coin to tackle the debt ceiling crisis, cash remains the reigning monarch in the world of payments. In a notable occurrence during her trip to the Bureau of Engraving and Printing in Fort Worth, Texas, in December, Treasury Secretary Janet L. Yellen made history by signing commemorative notes at the unveiling of a fresh series of dollar bills.
    \end{footnotesize} & {\footnotesize 1.574} \\
    \textbf{{\footnotesize }}  &     \begin{footnotesize}
As debates about digital currencies and the possibility of minting a trillion-dollar platinum coin to address the debt ceiling crisis capture headlines, cash may appear out of touch with the times. However, it continues to hold its position as the primary mode of payment in many regions worldwide. In December, Treasury Secretary Janet L. Yellen left her mark during a significant event at the Bureau of Engraving and Printing in Fort Worth, Texas, signing commemorative notes at the unveiling of a new batch of dollar bills.
    \end{footnotesize} & {\footnotesize 1.513} \\
\end{longtblr} 
\end{comment}
% ----------------------------------------------


\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/opt-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/opt-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt3-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt3-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/vicuna-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/vicuna-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/stablelm-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/stablelm-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/mpt-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/mpt-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/llama-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/llama-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/alpaca-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/alpaca-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt2-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt2-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/dolly-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/dolly-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/bloom-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/bloom-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t0-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t0-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/xlnet-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/xlnet-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

\begin{figure}[!htbp]
\centering
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t5-HP.pdf}
    \subcaption{blah}
\end{minipage}%
\hspace{0.5cm}
\begin{minipage}{.4\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t5-LP.pdf}
    \subcaption{blah}
\end{minipage}%
\caption{hist-line-perp-plots}
\label{fig:hist-line-perp-plot}
\end{figure}

% -----------------------------------------

\begin{comment}
\begin{figure*}[!htbp]
\centering
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt2-HP.pdf}
    \subcaption{GPT2-HP}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/dolly-HP.pdf}
    \subcaption{Dolly-HP}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/bloom-HP.pdf}
    \subcaption{BLOOM-HP}
\end{minipage}% 
\\
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/GPT2-LP.pdf}
    \subcaption{GPT2-LP}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/Dolly-LP.pdf}
    \subcaption{Dolly-LP}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/Bloom-LP.pdf}
    \subcaption{BLOOM-LP}
\end{minipage}%
\caption{hist-line-perp-plots for gpt2, Dolly, Bloom}
\label{fig:hist-line-perp-plot}
\end{figure*}
\end{comment}

% -----------------------------------------------------

\begin{figure*}[!htbp]
\centering
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t0-HP.pdf}
    \subcaption{T0-HP}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/xlnet-HP.pdf}
    \subcaption{XLNet-HP}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t5-HP.pdf}
    \subcaption{T5-HP}
\end{minipage}% 
\\
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t0-LP.pdf}
    \subcaption{T0-LP}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/xlnet-LP.pdf}
    \subcaption{XLNet-LP}
\end{minipage}%
\begin{minipage}{.3\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t5-LP.pdf}
    \subcaption{T5-LP}
\end{minipage}%
\caption{hist-line-perp-plots for t0, xlnet, t5}
\label{fig:hist-line-perp-plot}
\end{figure*}

% ----------------------------------------

%This combination proves to be highly effective in detecting and replacing high entropy words, ultimately leading to successful de-watermarking of the OPT-generated text. 
% \textcolor{red}{An important question that arises is whether there is a distinct winning combination among the 15 LLMs and which one to choose in real-life scenarios when we aim to de-watermark an AI-generated text in the wild. Our rigorous experiments suggest that the duo of (\texttt{albert-large-v2, distilroberta-base}) performs the best overall. To further support this claim, we provide results for the remaining 14 LLMs in Appendix \cref{sec:appendix}).}
% \mc{this red text here needs a rewrite.}

\begin{comment}

\textcolor{red}{show empirically which model is best for spotting high entropy tokens}
\textcolor{teal}{Method 1: To detect high entropy words based on their probability, one would need access to a language model that provides probability estimates for words. The general approach to identifying high entropy words using word probabilities can be summarized like below:}

% cite -  ATMAN: https://arxiv.org/pdf/2301.08110.pdf

% cite -https://arxiv.org/pdf/2303.11156.pdf

% move following detailed steps to appendix + shorten and add 1/2 lines

\textcolor{teal}{1. Choosing a specific language model or probability distribution one wants to work with. This could be a pre-trained language model like GPT-3 or any other model that provides word probability estimates.}



\textcolor{teal}{2. Tokenizing the text one wants to analyze into individual words or tokens.}

\textcolor{teal}{3. For each word/token in the text, querying the language model to obtain its probability estimate. This typically involves providing the context of the word in a sentence or surrounding context to get accurate probabilities.}

\textcolor{teal}{4. Comparing the probabilities of the words. Higher entropy words will have lower probabilities compared to lower entropy words. The greater the difference in probability among words, the higher the entropy.}

\textcolor{teal}{5. Setting a threshold to define what constitutes a high entropy word based on the probability distribution of the specific language model (In our case it was 40\%).} 

\textcolor{teal}{6. Filtering and identifying the words that fall below the threshold as high entropy words.}


\textbf{Masking high entropy words:}
\textcolor{red}{show empirically which model is best for masking high entropy tokens}
The technique for watermarking proposed in the Maryland paper \cite{tc-gpt} has an official website that can generate, watermark, and detect watermarked texts based on various LLMs, such as facebook/opt-6.7b, EleutherAI/gpt-neox-20b, bigscience/bloom, etc. However, there are some issues with the generation and detection technique. For example - 

1. The generation quality of texts with few sentences is weak.

2. \vjt{In cases where multiple paragraphs of watermarked text are combined into a single paragraph, the detector may fail to recognize it as watermarked text even if the original text was generated by the same website. However, it is worth noting that this issue only occurred with some texts and not all.}

Therefore, it is evident from the preceding discussion that the website proposed by the Maryland paper \cite{tc-gpt} is not infallible and sometimes fails to detect AI-generated texts.
\end{comment}



\begin{comment}
\begin{table*}[!ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{0.2\textwidth} | p{0.8\textwidth}|} %{ll}
\hline
\textbf{Prompt}            & {Will the next great writer be a robot? }
    \\ \hline
\textbf{Watermarked text} & {I'm \colorbox{pink}{very skeptical} that the next "great writer" is going to be a robot, \colorbox{pink}{or} that they'll be \colorbox{pink}{much} more effective at \colorbox{pink}{expressing the} subtleties and depths of \colorbox{pink}{human} thought than a human is.
However, what is \colorbox{pink}{most} interesting is the role that the \colorbox{pink}{Internet could} play in bringing these "robot" writers into the public eye. If I could (and I'm \colorbox{pink}{very} excited by this possibility), I would pay a \colorbox{pink}{small monthly} fee to \colorbox{pink}{read well-written}...}
 \\ \hline
\textbf{De-Watermarked text by replacing high-entropy words}              & {I'm \colorbox{green}{somewhat} skeptical that the next "great writer" is going to be a robot, \colorbox{green}{given} that they'll be \colorbox{green}{far} more effective at \colorbox{green}{grasping deeper} subtleties and depths of philosophical thought than a robot is. However, what is \colorbox{green}{particularly} interesting is the role that the Internet \colorbox{green}{may} play in bringing new great writers into the public eye. If I did (and I'm \colorbox{green}{extremely} excited by this possibility), I would pay a \colorbox{green}{hefty subscription} fee to \colorbox{green}{publish  something}}...
 \\ \hline
\textbf{De-Watermarked text by paraphrasing}              & I have \colorbox{cyan}{serious doubts} about the possibility of a robot becoming the next \colorbox{cyan}{exceptional writer} and \colorbox{cyan}{surpassing humans} in expressing the nuances and profoundness of human thoughts. Nevertheless, what \colorbox{cyan}{fascinates} me the most is the potential impact of the \colorbox{cyan}{Internet in showcasing} these "robot" writers to the general public. The idea of being able to pay a \colorbox{cyan}{nominal monthly} subscription fee to access \colorbox{cyan}{impeccably written} and carefully refined works \colorbox{cyan}{truly} thrills me...
\\ \hline
\end{tabular}%
}
\caption{De-Watermarking by replacing high-entropy words}
\label{tab:dewatermarking-m1}
\end{table*}
\end{comment}


\begin{comment}
\begin{table}[!ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{0.28\columnwidth} | p{0.7\columnwidth}|} %{ll}
\hline
\textbf{Prompt}            & {Will the next great writer be a robot?\n\nAt the PEN America Literary Awards, David Sedaris, Judith Thurman and other human writers discussed the role that AI could play in literature.}
    \\ \hline
\textbf{Watermarked text} & {I'm \colorbox{pink}{very skeptical} that the next "great writer" is going to be a robot, \colorbox{pink}{or} that they'll be \colorbox{pink}{much} more effective at \colorbox{pink}{expressing the} subtleties and depths of \colorbox{pink}{human} thought than a human is.
However, what is \colorbox{pink}{most} interesting is the role that the \colorbox{pink}{Internet could} play in bringing these "robot" writers into the public eye. If I could (and I'm \colorbox{pink}{very} excited by this possibility), I would pay a \colorbox{pink}{small monthly} fee to \colorbox{pink}{read well-written}, \colorbox{pink}{well-re}...}
 \\ \hline
\textbf{De-Watermarked text}              & I have \colorbox{green}{serious doubts} about the possibility of a robot becoming the next \colorbox{green}{exceptional writer} and surpassing \colorbox{green}{humans} in expressing the nuances and profoundness of human thoughts. Nevertheless, what \colorbox{green}{fascinates} me the most is the potential impact of the Internet in showcasing these "robot" writers to the general public. The idea of being able to pay a \colorbox{green}{nominal monthly} subscription fee to access \colorbox{green}{impeccably written} and carefully refined works \colorbox{green}{truly} thrills me.
\\ \hline
\end{tabular}%
}
\caption{De-Watermarking by paraphrasing}
\label{tab:dewatermarking-m1}
\end{table}
\end{comment}



\begin{comment}
\begin{table*}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|p{0.85in}|p{2.15in}|} %{ll}
\hline
\textbf{Prompt}            & [insert NYT tweet]    \\ \hline
\textbf{Watermarked text} & [insert highlighted watermarks] \\ \hline
\textbf{De-Watermarked text}              & [insert highlighted replacements] 
\\ \hline
\end{tabular}%
}
\caption{De-Watermarking by paraphrasing}
\label{tab:dewatermarking-m2}
%\end{table}
% \end{minipage}
\end{table*}
\end{comment}

%Now, if we base our de-watermarking experiments on this website, we have attempted 4 masking LLMs (albert-large-v2, xlm-roberta-large, bert-base-uncased, distilroberta-base) to detect and replace high entropy words. We tested each of the model for detecting high entropy words by iterating over each masked word in the entire watermarked paragraph. The high entropy words were determined based on the likelihood of the masked word occurring. If the probability was less than 40 percent, the word was identified as having a high entropy. After identifying all the words with high entropy, we replaced them with a word from the same or another language model. We basically made a matrix of detecting and replacing watermarked words with the above mentioned 4 LLMs creating a 16 combination technique.


\begin{comment}
\begin{figure}[htp!]
    \centering
    \includegraphics[width=\columnwidth]{img/De-WM-best5.png}
    \caption{Accuracy of the best five LLM combinations}
    \label{fig:my_label}
\end{figure}    
\end{comment}

% \textbf{Reverse engineering to find out random deletion series}
%\textcolor{orange}{We can now empirically conclude that given a watermarked text from any of the common LLMs, simply by replacing the high entropy words, we are able to de-watermark the black-listed tokens. Thus, making it impossible to detect whether a text is generated by AI or not through the watermarking technique.}

%We  conduct an extensive study on the qualitative and quantitative aspects of automatic paraphrasing.
%One possible solution to de-watermarking is to paraphrase the content generated by the LLM, either as a whole or on a sentence-by-sentence basis. However, a crucial question arises: will the same system \cite{tc-gpt} be able to detect the de-watermarked content? To answer this question empirically,

% ---------------------------

\begin{comment}
\vspace{-2mm}
\begin{figure}[h]
    \centering
\includegraphics[width=\columnwidth, height=20mm]{img/sentence_level_perplexity.png}
\caption{Perplexity estimation for OPT sentence by sentence.}
    \label{fig:entropy}
\end{figure}
\vspace{-1mm}
\end{comment}
%~\ref{eqn:perplexity_sentence_wise}.
%\textcolor{teal}{The meaning of 's' in the equations is unclear for both PE and BE. It would be better to add what 's' stands for.}
%, and variations of perplexity scores across sentences should be relatively lower for AI-generated text. The hypothesis is incomplete and only validated with GPT model, that too when the input text is at least \acb{250} characters long. 
\begin{comment}
    \vspace{-5mm}
    \begin{equation}
    \label{eqn:perplexity_overall}
    log p_{\Theta}(h_{text})-log p_{\Theta}(AI_{text}) \geq 0
    \end{equation}
    \vspace{-6mm}
    %
    \begin{equation}
    \label{eqn:perplexity_sentence_wise}
    \resizebox{0.9\hsize}{!}{%
    log p_{\Theta}[\Sigma_{k=1}^{n-1}(|s_{h}^{k}-s_{h}^{k+1}|)]-log p_{\Theta}[\Sigma_{k=1}^{n-1}(|s_{AI}^{k}-s_{AI}^{k+1}|)] \geq 0
    }
    \end{equation}
\end{comment}

% --------------------------

\begin{comment}
The final dataset used for \textbf{CT}$^2$ and ADI consists of 1500K data points.
The development of \textbf{CT}$^2$ and ADI required parallel data, specifically human-written text and AI-generated text on the same topic. We selected \href{https://twitter.com/nytimes}{The New York Times' Twitter handle} as our data source for several reasons -  a) Firstly, the handle comprises approximately 510.4K tweets that cover a wide range of topics. For this paper, we chose a subset of 100K tweets. b) Secondly, the New York Times is renowned for its reliability and credibility. c) Thirdly, all the tweets from this source include URLs that lead to the corresponding human-written news articles. d) Lastly, despite Twitter's reputation for noisy language, the tweets from the New York Times are skillfully composed by professional journalists, free from grammatical errors. These tweets serve as prompts for the 15 LLMs, with any noise-related elements such as hashtags and mentions removed during the cleaning process.    
\end{comment}
 

\begin{comment}
\textcolor{teal}{`The New York Times', being one of the most authentic news sources in the world, has been used to create the AI generated text dataset. The process of creating the dataset can be summarized as follows: \\ 
1. Twitter data scrapping was utilized to extract about 393k tweets and their original human written story spanning from 2007 to 2021. \\
2. The tweets were then used to create AI Generated text using 15 LLMs (GPT 4, GPT 3.5, GPT 3, GPT 2, MPT, OPT, LLaMA, BLOOM, Alpaca, Vicuna, Dolly, StableLM, XLNet, T5 and T0). \\
3. There were some punctuation errors while scrapping the data, hence, they were cleaned for both human generated and AI generated texts. \\
4. The links to the NYT website was always present in the tweet and those were also removed to keep the dataset URL free.}

\textcolor{teal}{The reasons for choosing the 15 LLMs are primarily because they are open source and the variations they can create due to their different nature. Moreover, the watermarking website featured 6 LLMs from the LLM list that this paper has provided. Therefore, this study closely aligns with the work of the Maryland paper.}
\end{comment}

% ------------------------------------

\begin{comment}
\begin{table*}[!ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ | p{0.06\textwidth} |
                   p{0.55\textwidth} |
                   p{0.02\textwidth} |
                   p{0.02\textwidth} |
                   p{0.55\textwidth} |
                   p{0.02\textwidth} |
                   p{0.02\textwidth} |}
\toprule
 &
   &
  \textbf{\rotatebox[origin=c]{90}{Z-score}} &
  \textbf{\rotatebox[origin=c]{90}{p-value}} &
   &
 \textbf{\rotatebox[origin=c]{90}{Z-score}} &
 \textbf{\rotatebox[origin=c]{90}{p-value}} \\ \midrule
\textbf{Prompt} &
  \textit{Will the next great writer be a robot?} &
   &
   &
 \textit{Detecting AI-generated text is challenging but not impossible. Ongoing efforts improve accuracy and uphold transparency.} &
   &
   \\ \hline
\textbf{\rotatebox[origin=r]{90}{\parbox[c]{2cm}{\centering Watermarked text}}}
    &
    {I'm \colorbox{pink}{very skeptical} that the next "great writer" is going to be a robot, \colorbox{pink}{or} that they'll be \colorbox{pink}{much} more effective at \colorbox{pink}{expressing the} subtleties and depths of \colorbox{pink}{human} thought than a human is. However, what is \colorbox{pink}{most} interesting is the role that the \colorbox{pink}{Internet could} play in bringing these "robot" writers into the public eye. If I could (and I'm \colorbox{pink}{very} excited by this possibility), I would pay a \colorbox{pink}{small monthly} fee to \colorbox{pink}{read well-written}...}
   & \rotatebox[origin=c]{90}{\parbox[r]{1.5cm}{\centering 4.24}}
   & \rotatebox[origin=c]{90}{\parbox[r]{2cm}{\centering 1.1e-05}}
   &
   AI has made \colorbox{pink}{great} strides, and the potential of these technologies to \colorbox{pink}{improve} our lives is enormous. However, AI \colorbox{pink}{also} can pose ethical and \colorbox{pink}{social} challenges.
In this article, we discuss some of the ways AI text analysis is used to generate \colorbox{pink}{harmful language}, and the \colorbox{pink}{work} being undertaken to detect and prevent it. We also discuss some \colorbox{pink}{recent work} aimed at \colorbox{pink}{ensuring transparency} and interoperability in text analysis. 
& \rotatebox[origin=c]{90}{\parbox[r]{1.5cm}{\centering 5.06}}
   & \rotatebox[origin=c]{90}{\parbox[r]{1.5cm}{\centering 2.06e-07}}
   \\ \hline
\textbf{\rotatebox[origin=r]{90}{\parbox[c]{5cm}{\centering De-Watermarked text by replacing high-entropy words}}} &
    {I'm \colorbox{green}{somewhat} skeptical that the next "great writer" is going to be a robot, \colorbox{green}{given} that they'll be \colorbox{green}{far} more effective at \colorbox{green}{grasping deeper} subtleties and depths of philosophical thought than a robot is. However, what is \colorbox{green}{particularly} interesting is the role that the Internet \colorbox{green}{may} play in bringing new great writers into the public eye. If I did (and I'm \colorbox{green}{extremely} excited by this possibility), I would pay a \colorbox{green}{hefty subscription} fee to \colorbox{green}{publish  something}}...
   & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 1.76 \textcolor{red}{[58.5\% \Downarrow}]}}
   &     \rotatebox[origin=c]{90}{\parbox[r]{4cm}{\centering 0.039\textcolor{red}{[3.5e05\% \Uparrow}]}}
   &
   AI has made \colorbox{green}{tremendous} strides and the potential of these technologies to \colorbox{green}{transform} our lives is exciting However, AI \colorbox{green}{manipulation} can pose ethical and \colorbox{green}{legal} challenges. In this article, we discuss some of the ways AI text analysis is used to generate \colorbox{green}{artificial speech} and the \colorbox{green}{measures} being undertaken to detect and prevent it. We also discuss some \colorbox{green}{important steps} aimed at \colorbox{green}{improving accuracy} and interoperability in text analysis. & 
    \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 3.72 \textcolor{red}{[26.48\% \Downarrow}]}}
    
   &     \rotatebox[origin=c]{90}{\parbox[r]{4cm}{\centering 9.96e-05 \textcolor{red}{[4.8e04\% \Uparrow}]}}
   \\ \hline
\textbf{\rotatebox[origin=r]{90}{\parbox[c]{5cm}{\centering De-Watermarked text by paraphrasing}}} &
    I have \colorbox{cyan}{serious doubts} about the possibility of a robot becoming the next \colorbox{cyan}{exceptional writer} and \colorbox{cyan}{surpassing humans} in expressing the nuances and profoundness of human thoughts. Nevertheless, what \colorbox{cyan}{fascinates} me the most is the potential impact of the \colorbox{cyan}{Internet in showcasing} these "robot" writers to the general public. The idea of being able to pay a \colorbox{cyan}{nominal monthly} subscription fee to access \colorbox{cyan}{impeccably written} and carefully refined works \colorbox{cyan}{truly} thrills me...
   & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering -0.542 \textcolor{red}{[112.78\% \Downarrow}]}}
   & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 0.706 \textcolor{red}{[6.4e6\% \Uparrow}]}}

   &
The \colorbox{cyan}{advancements} in AI have been significant and hold immense potential for \colorbox{cyan}{enhancing} our daily lives. Nevertheless, there are ethical and \colorbox{cyan}{societal} \colorbox{cyan}{concerns} that come with the use of AI. This piece delves into the \colorbox{cyan}{negative impact} of AI-generated language and the \colorbox{cyan}{measures being taken} to identify and prevent it. Additionally, we explore \colorbox{cyan}{recent efforts} to \colorbox{cyan}{promote transparency} and compatibility in text analysis.  & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 0.593 \textcolor{red}{[88.28\% \Downarrow}]}}
   & \rotatebox[origin=c]{90}{\parbox[r]{3cm}{\centering 0.276 \textcolor{red}{[1.3e8\% \Uparrow}]}}

   \\ \bottomrule
\end{tabular}%
}
\caption{}
\label{tab:dewatermarking_table}
\end{table*}    
\end{comment}

% -------------------------------------------------
\begin{comment}
\begin{table}[!ht]
\begin{tabular}{ccccccc}
\hline
\multirow{3}{*}{Models} & \multicolumn{6}{c}{Paraphrase}                                                      \\ \cline{2-7} 
                        & \multicolumn{2}{c}{GPT-3} & \multicolumn{2}{c}{Pegasus} & \multicolumn{2}{c}{T5}    \\ \cline{2-7} 
                        & v1             & v2       & v1              & v2        & v1                   & v2 \\ \hline
OPT                     & 100.0\%        &          & 100.0\%         &           & \multicolumn{1}{l}{} &    \\
\hline
\end{tabular}
\caption{blah}
\label{tab:para-dewm}
\end{table}
\end{comment}




% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}

% \begin{table}[h!]
% \centering
% \resizebox{0.5\columnwidth}{!}{%
% \begin{tabular}{@{}ll@{}}
% \toprule
% \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Paraphrasing\\ techniques\end{tabular}} & \multicolumn{1}{c}{Acc.} \\ \midrule
% Pegasus \cite{zhang2020pegasus}                  & 75.32 \\
% T5 (T5-Large) \cite{raffel2020exploring}         & 77.86 \\
% GPT-3 \cite{brown2020language}                   & 80.32 \\ \bottomrule
% \end{tabular}%
% }
% \caption{}
% \label{tab:my-table}
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}

% ---------------------------------------------

%As indicated in Table \cref{tab:winning_combination_opt}, our experiments empirical \textcolor{red}{evidence that the watermarking applied to AI-generated text} can be easily circumvented. 
%We present a comprehensive study on the utilization of two methods for de-watermarking.
%the tokens making the technique ineffective.


%\textcolor{teal}{There has been a recent update to the watermarking strategy in which \cite{kirchenbauer2023reliability} added additional logic implementing a wider variety of seeding schemes and alternative detection strategies. Extended versions of the classes in the watermarking directory depend on this logic. However, we applied our dewatermarking technique to the newly generated watermarked text using OPT model and found out that our techniques are still robust enough to successfully dewatermark with good accuracies. To showcase the performance of the dewatermarking technique on this updated watermarking strategy, the v2 of table 3 can be portrayed.}


% -----------------------------------------------
% \input{nlc_figure}

%The hypothesis put forward in \cite{mitchell2023detectgpt} suggests that the perturbation patterns of AI-written text should align with the negative log-likelihood region. However, this observation is not supported by the results presented here. To strengthen our conclusions, we calculated the standard deviation, mean, and entropy, and performed a statistical validity test in the form of a p-test. The findings are reported in Table ~\cref{tab:perp-burst-nlc-compile}. Therefore, our argument is that \acb{while NLL serves as a valid `signal' for attribution, it is not a robust and conclusive differentiator between human and AI-generated text.}


%DetectGPT \cite{mitchell2023detectgpt} utilizes the generation of log-probabilities for textual analysis. It leverages the difference in perturbation discrepancies between machine-generated and human-written text to detect the origin of a given piece of text. When a language model produces text, each individual token is assigned a conditional probability based on the preceding tokens. These conditional probabilities are then multiplied together to derive the joint probability for the entire text. To determine the origin of the text, DetectGPT introduces perturbations. If the probability of the perturbed text significantly decreases compared to the original text, it is deemed to be AI-generated. Conversely, if the probability remains roughly the same, the text is considered to be human-generated. For instance, let's consider the following two sentences as an example:




% Original input: "This sentence is generated by an AI or human" => log-probability \#1. \\
% Perturbed input: "This writing is created by an AI or person" => log-probability \#2

%


\begin{comment}
\begin{multicols}{2}
\begin{strip}
\begin{align}
\resizebox{\textwidth}{!}{ADI_x=\frac{100}{U}*\frac{1}{2}\left[(1-\mu_H^{plx}) * \{\sum_{x=1}^U\left(log p_u^{i}-log p_u^{i+1}\right)+\delta_1(x)\}+(1-\mu_H^{brsty}) * \{\sum_{x=1}^U\left(log p_u^{i+(i+1)+(i+2)}-log p_u^{(i+3)+(i+4)+(i+5)}\right)+\delta_2(x)\}\right]}
\label{eq:eq1}
\end{align}
\end{strip}
\end{multicols}



\begin{multicols}{2}
\begin{strip}
\begin{align}
\resizebox{\textwidth}{!}{ADI_x=\frac{100}{2} * [\{\delta_1(x)*\frac{\left( P_t-L_H^{plx}\right)}{\left(1-\mu_H^{plx}\right)}\}+\{\delta_2(x)*\frac{\left(B_t-L_H^{brsty}\right)}{\left(1-\mu_H^{brsty}\right)}\}]}
\label{eq:eq1}
\end{align}
\end{strip}
\end{multicols}
\end{comment}

%Negative log likelihood scores were computed for text generated by both AI and human sources. A t-test was conducted to examine the significance of these scores. The results of the t-test indicated a significant outcome; however, the p-values obtained were exceptionally low. To ensure that the t-test assumption of normality was met, the distributions of the scores were assessed. It was determined that the distributions did not adhere to the normality assumption, rendering the t-test inappropriate for further analysis. Therefore, a bootstrap test, which is designed for non-normal distributions, was conducted. The results of the bootstrap test showed that the test outcome was not significant.

\begin{comment}
    \begin{table}[htp]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}clllll@{}}
\toprule
\multicolumn{2}{l}{\textbf{Models}} & \textbf{AI Text} & \textbf{Human Text} & \textbf{$\sigma_{AI}$ - $\sigma_{Human}$} & \textbf{Bootstrap P-Value} \\
\midrule
\multirow{2}{*}{\textbf{GPT-2}}  & \textbf{$\mu$}  & 1.456  & 1.495  & 0.034 & 0.4969 \\
    & \textbf{$\sigma$} & 0.104   & 0.070  &  &  \\
    \cmidrule(l){2-6} 
\multirow{2}{*}{\textbf{OPT}}  & \textbf{$\mu$}  & 2.488  & 2.763  & -0.112 & 0.4918 \\
    & \textbf{$\sigma$} & 0.346   & 0.458  &  &  \\ 
    \cmidrule(l){2-6}
\multirow{2}{*}{\textbf{Bloom}}  & \textbf{$\mu$}  & 3.084  & 3.279  & -0.095 & 0.5034 \\
    & \textbf{$\sigma$} & 0.381  & 0.476  &  &  \\
\toprule
\end{tabular}%
}
\caption{Statistical measures of Negative Log Likelihood in AI vs Human Text for Models GPT-2, OPT and Bloom.}
\label{table:opt-xlnet-stat}
\end{table}
\end{comment}


\begin{comment}
\begin{figure}[htp]
    \centering
\includegraphics[width=\columnwidth]{img/ADI.pdf}
                \caption{ADI. \textcolor{red}{add hyperparameters like Vipula did, and size of LLM}}
    \label{fig:ADI}
\end{figure}
\end{comment}


%\input{ADI_table}


%In particular, by identifying LLMs that surpass an ADI threshold, appropriate ownership attribution could be enforced using policy control and regulation.









%Watermarking is a protective measure that safeguards AI-generated text from being detected, thereby preventing possible misuse. In addition to watermarking, two significant families of detection methods have been proposed, namely negative log-likelihood and perplexity and brustiness estimation. We have discussed the advantages and disadvantages of these methods so far. Advancements in LLMs have accelerated significantly, and it's expected that we may witness the emergence of even better LLMs in the near future that can generate text which is difficult to detect using the aforementioned methods. However, this also means that newer methods for AI-generated text detection will continue to be an attractive area for researchers, and as a result, we can expect to see the proposal for better detection methods. The AI Detectability Index (ADI) is defined to quantify the detectability of an LLM's generated text by a system and can also serve as a risk measurement index. Practitioners can use the ADI score to select the model that best suits their downstream task. 




% \ac{Further explanation is required to elaborate on the specific components and calculations involved in the formula. Please provide the necessary information to explain the formula in question.}



\begin{comment}
\begin{figure}[htp]
    \centering
\includegraphics[width=\columnwidth]{img/ADI.pdf}
                \caption{ADI. \textcolor{red}{add hyperparameters like Vipula did, and size of LLM}}
    \label{fig:ADI}
\end{figure}
\end{comment}


%\input{ADI_table}




\begin{comment}
\begin{table}[htp!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{1}{l}{\textbf{LLMS}}               & \multicolumn{1}{l}{\textbf{ADI}} \\ \midrule
PanGu-Σ                                         &                                  \\
GPT-4                                           &                                  \\
Falcon                                          &                                  \\
Cerebras-GPT                                    &                                  \\
BloombergGPT                                    &                                  \\
LLaMA (Large Language Model Meta AI)            &                                  \\
Galactica                                       &                                  \\
AlexaTM (Teacher Models)                        &                                  \\
BLOOM                                           &                                  \\
YaLM 100B                                       &                                  \\
Minerva                                         &                                  \\
OPT (Open Pretrained Transformer)               &                                  \\
PaLM (Pathways Language Model)                  &                                  \\
Chinchilla                                      &                                  \\
GPT-NeoX                                        &                                  \\
LaMDA (Language Models for Dialog Applications) &                                  \\
Gopher                                          &                                  \\
GLaM (Generalist Language Model)                &                                  \\
Ernie 3.0 Titan                                 &                                  \\
Claude{[}45{]}                                  &                                  \\
Megatron-Turing NLG                             &                                  \\
GPT-J                                           &                                  \\
GPT-Neo                                         &                                  \\
GPT-3                                           &                                  \\
XLNet                                           &                                  \\
GPT-2                                           &                                  \\
BERT                                            &                                  \\ \bottomrule
\end{tabular}%
}
\caption{AI Detectability Index (ADI) scores for 27 LLM}
\label{tab:ADI}
\end{table}
\end{comment}


%\adas{However, a contrasting perspective is presented by \cite{chakraborty2023possibilities} on this matter. The study suggests that with a sufficient number of sample points from a specific LLM, it is possible to develop improved AGTD techniques tailored to a particular LLM. However, when it comes to handling text found in real-world scenarios, the question of which specific AGTD techniques to use for the particular case remains unanswered. Furthermore, the study does not provide empirical evidence or specify the required sample size, thus leaving the claim as a hypothesis at this stage. Additionally, the authors propose that employing techniques such as watermarking can alter the distribution of AI-generated text, making it distinguishable from the distribution of human-generated text and therefore detectable. However, the authors did not provide any empirical evidence to support this hypothesis.}


% -------------------------------------------------
%refers to the tendency of a term to reappear in a document after its initial usage. This means that subsequent occurrences of a word carry less importance compared to its first occurrence. AI models have made impressive advancements in replicating human writing styles, including the phenomenon of burstiness. However, they may occasionally fall short in capturing the same degree of variation, emotional depth, and contextual comprehension that is present in human writing. In contrast, human-authored text tends to exhibit a greater range of bursts, influenced by personal style, individual experiences, and creative expression. These differences emerge due to the contrasting methodologies employed by AI models and humans in generating language. AI models rely on statistical patterns acquired through learning, whereas humans utilize personal experiences and linguistic capabilities to produce text.

%Prior research \cite{rychly2011words, cummins2017modelling} has indicated that there are distinct variations in burstiness characteristics between text generated by AI and text authored by humans. Calculating burstiness involves converting the text into a sequence of numerical tokens using the tokenizer. To enhance computational efficiency, both the model and tokenizer are optimized for utilization on a graphics processing unit (GPU) when available. The token sequence is also prepared for GPU computation. The model then generates the probabilities of the next word for each token in the text. These probabilities are further processed and organized as numerical values within an array. By quantifying the variation in these probabilities, we derive the burstiness score, representing the level of fluctuation in the occurrence of events within the text. The burstiness score is obtained by calculating the average value of this variation. However, we found that the burstiness scores of AI-written text and human-written text were very similar. This means that the way events are distributed within the text is alike for both AI and human writing, even though there are still some differences. 

\begin{comment}
\begin{table}[htp]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}clcc@{}}
\toprule
\multicolumn{2}{c}{\textbf{Models}} & \textbf{Human Text} & \textbf{AI Text} \\
\midrule
\multirow{2}{*}{\textbf{OPT}}  & \textbf{$\mu$}  & 4.09279e-06  & 1.02997e-08 \\
    % & \textbf{variance}       & 0.357  & 0.492 \\
    & \textbf{$\sigma$} & 7.63874e-07  & 1.81573e-09 \\ 
    \cmidrule(l){3-4} 
\multirow{2}{*}{\textbf{GPT2}} & \textbf{$\mu$}  & 3.40542e-06  & 3.05180e-06   \\
    % & \textbf{variance}       & 0.505  & 0.904  \\
    & \textbf{$\sigma$} & 5.71742e-07 & 5.95274e-07  \\ 
\toprule
\end{tabular}%
}
\caption{Statistical measures of Burstiness score in AI vs Human Text for Models OPT and GPT2}
\label{table:opt-gpt2-stat}
\end{table}   
\end{comment}




% Additionally, to provide a clearer picture, we also report the mean and standard deviation of the perplexity measurements, the rest are in the appendix \ref{sec:appendix}.

%This analysis provides insights into the varying levels of detectability exhibited by different-sized language models, highlighting the importance of model size in determining the robustness of the generated text.


%\vspace{-2mm}

% \begin{figure}
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.4\linewidth]{img/gpt-perp-histplot.png}
%   \caption{A subfigure}
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=.4\linewidth]{img/opt-perp-histplot.png}
%   \caption{A subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{A figure with two subfigures}
% \label{fig:test}
% \end{figure}

%for now, not using subfigure

   


%\includegraphics[width=\columnwidth]{img/gpt_perplexity.png}

%Within the scope of this discussion, two pertinent questions remain unanswered. The first question pertains to the estimation of perplexity while accounting for potential variations from one sentence to another for human-written text and AI-generated text. The second question revolves around calculating perplexity specifically for non-open source Language Models (LLMs) like GPT4. In terms of understanding perplexity variations at the sentence level, we estimate entropy using the following equation: $log p_{\Theta}[\Sigma_{k=1}^{n}(|s_{h}^{k}-s_{h}^{k+1}|)]-log p_{\Theta}[\Sigma_{k=1}^{n}(|s_{AI}^{k}-s_{AI}^{k+1}|)] \geq 0$. 
%\ac{Is this the intended equation here? This is an inequality, but we need a formula for entropy here.}






%used in natural language processing to evaluate the performance of language models. A language model trained on the human-written text will likely have a lower perplexity score, indicating better performance in predicting the next word or sequence of words. AI-written text is generated by language models that have been trained on large datasets of human-written text which results in a higher perplexity score. The perplexity score for human-written text is generally lower than that for AI-written text because the human-written text is more coherent, contextually accurate, and grammatically correct, making it easier for language models to predict the next word or sequence of words.

%The perplexity of a text can be calculated using the following formula:

%\[
%\text{{Perplexity}} = e^{-\frac{1}{N} \sum_{i=1}^{N} \log_2 p(w_i)}
%\]


%GPTZero \cite{gptzeroapi} computes perplexity values. The perplexity is related to the log probability of the text mentioned for DetectGPT above. The perplexity is the exponent of the negative log probability. So, the lower the perplexity, the less random the text. Large language models learn to maximize the text probability, which means minimizing the negative log probability, which in turn means minimizing the perplexity. GPTZero then assumes that text with lower perplexity is more likely generated by an AI.

%We take an example of human-generated text from our dataset and feed it to the GPT model to check whether or not it identifies the text as human-generated.

%\emph{\textcolor{gray}{“The Northeast is forecast to get sleet and snow starting on Monday and continuing into Tuesday after a mild winter in which the region has been spared the kinds of snowstorms that have affected other parts of the United States over the past week. Four to more than six inches of snow are possible in interior portions of the Northeast, including New Jersey, the Lower Hudson Valley and southern Connecticut, with the first flakes starting late on Monday, according to the National Weather Service in New York. Snow-covered roads are expected to make for a slow commute on Monday evening and Tuesday morning. One to three inches of wet snow and sleet could fall in northern areas of New York City, Long Island and parts of New Jersey, from Newark to Paramus, on Monday evening until early Tuesday before the precipitation transitions to rain in the city and along the coast, forecasters said.”}}

%The text generation model being used has certain limitations, such as a character limit of 250 characters. This can pose a challenge when generating longer texts, as the input text will be truncated, and the generated text may not accurately reflect the intended meaning. Additionally, although the input text is taken from a reliable source, the NYTimes story, the model is incorrectly identifying it as AI-generated text. This highlights the fact that the model's identification and classification mechanisms are not perfect and may be influenced by various factors. The model's classification is based on perplexity, which is a metric that estimates how well the model can predict the next word in a sequence of text. However, perplexity estimation is not an absolute method for distinguishing between human-generated and AI-generated content, as other factors such as style, tone, and coherence may also be important. Therefore, it is important to approach the model's results with some degree of caution and take into account other factors when assessing the authenticity and quality of the generated text.

\begin{comment}
\begin{table}[]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{clcc}
\toprule
\multicolumn{2}{c}{\textbf{Models}} & \textbf{AI Text} & \textbf{Human Text} \\ \toprule
\multirow{2}{*}{\textbf{GPT-2}} & \textbf{$\mu$} & 418.054 & 484.022 \\  
 & \textbf{$\sigma$} & 1090.609 & 1089.403 \\
 % & \textbf{$\sigma_{AI}$ - $\sigma$_{human}} & 1090.609 - 1089.403 & 00 \\
 \hline
\multirow{2}{*}{\textbf{OPT}} & \textbf{$\mu$} & 451.521 & 402.928 \\  
 & \textbf{$\sigma$} & 2832.363 & 897.251 \\ \hline
\multirow{2}{*}{\textbf{BLOOM}} & \textbf{$\mu$} & 941.110 & 1504.797 \\ 
 & \textbf{$\sigma$} & 5109.447 & 6855.744 \\ \hline
\multirow{2}{*}{\textbf{XLNET}} & \textbf{$\mu$} & 879.782 & 2772.043 \\  
 & \textbf{$\sigma$} & 4012.784 & 7855.392 \\ \bottomrule
\end{tabular}
}
\caption{Statistical measures of Perplexity for AI vs Human Text in Models GPT-2, OPT, BLOOM, and XLNet.}
\label{table: gpt-opt-bloom-xlnet-perp stats}
\end{table}
\end{comment}
% perplexity table include range (sd diff), bootstrap test, p-test etc 
% repeat same table with burstiness scores

%The perplexity mean and standard deviations when calculated on models like GPT-2, OPT, BLOOM are nearly the same (Table \ref{tab:perp-burst-nlc-compile}), hence the range cannot be determined. There are a number of reasons why human and AI written text may have identical perplexity scores and entropies. The enormous volumes of human-written text are used to train AI models, which could cause the language produced by AI to resemble human-written text in terms of both structure and style. Although the mean and standard deviation values for smaller language models like XLNet are similar just like those of larger language models such as GPT-2, OPT, and BLOOM, they exhibit a greater disparity between the perplexity scores of AI-generated text and human-generated text. In contrast, the mean and standard deviation values for GPT-2, OPT, and BLOOM demonstrate less variation between the perplexity scores of AI-generated and human-generated text. \textcolor{red}{(possible reasons??) The mean and standard deviations of larger language models like GPT-2, OPT, and BLOOM can have very similar numbers for AI-generated texts and human-generated texts due to the high capacity of these models to learn and replicate the linguistic patterns of human language. When trained on a large corpus of text, these models can capture the statistical regularities of language, including patterns of syntax, vocabulary, and semantics. As a result, the generated text from these models can be very similar to human-generated text in terms of these linguistic features, resulting in similar mean and standard deviation values for AI and human-generated texts. Additionally, these models are trained on a large and diverse dataset of text, which can include a range of writing styles and genres. This means that the models can generate text that mimics the patterns and nuances of different types of writing, from news articles to creative fiction. This diversity can further contribute to the similarities in mean and standard deviation values between AI-generated and human-generated text.} 
%\textcolor{blue}{In this study, we utilized both the t-test and the bootstrap test to comprehensively assess the differences between AI and human-generated text in terms of perplexity. The t-test allowed us to compare the means of the two groups and determine whether there was a statistically significant distinction between them. By comparing the t-statistic to a t-distribution, we calculated the p-value, which indicated the probability of observing a difference in perplexity as large or larger than the one observed, assuming no true difference between AI and human text. In addition to the t-test, we employed the bootstrap test to further enhance the robustness of our analysis, considering the large size of our dataset. We computed the bootstrap p-value. By comparing the observed perplexity difference to the distribution of bootstrap samples, we estimated the probability of observing a difference as large or larger than the one we observed if there was no true distinction between AI and human text. This bootstrap p-value allowed us to assess the statistical significance of the perplexity differences, providing additional evidence to support our conclusions.}AI models also produce text with similar perplexity scores and entropy values to human-written language since they are built to anticipate the next word in a phrase based on the context of the preceding ones. The scores may be being comparable, but the quality and coherence of content produced by AI models and that produced by humans varies. 



%Since the language models used to generate both human-written text and AI-written text are comparable, their data points— words, phrases, and sentences— are probably distributed similarly. This indicates that for both forms of text, the discrepancies between each data point and the dataset's mean are probably going to be similar.


%\textcolor{blue}{We argue it could easily be learned what are the thresholds of these perplexity values and could easily be reverse-engineered to fool the system. We present our experiments.}

%\vspace{-4mm}

\begin{comment}
\begin{table*}[!htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllllllllllllll@{}}
\toprule
LLMs   &            & \multicolumn{5}{l}{Perplexity} & \multicolumn{5}{l}{Burstiness} & \multicolumn{5}{l}{NLC}      \\ \midrule
       &                       & Human  & AI  & Ent$_H$ & Ent$_{AI}$ & b-value & Human  & AI  & Ent$_H$ & Ent$_{AI}$ & b-value & Human & AI & Ent$_H$ & Ent$_{AI}$ & b-value \\
GPT 4 \cite{openai2023gpt4}  & \mu    &   122.839   &     &     &   &        &   -0.3001     &     & &        &        &     4.160  &    &  &      &        \\
       & \sigma &    58.541    &     &   &     &        &    0.26164    &     &    &    &        &   0.336     &    &    &    &        \\
GPT 3.5 \cite{chen2023robust}  & \mu    &   122.839    &  56.558   & 4.276 & 2.856     &  0.506      &   -0.3001     &  0.1213   & 6.119  &  6.641    &    0.4945    &   4.160    & 3.386   & 4.301  & 2.867    &    0.499    \\
       & \sigma &    58.541    & 50.002    &   &     &        &  0.26164      &  0.3434   &      &  &        &    0.336   & 0.551   &  &      &        \\
OPT \cite{zhang2022opt}  & \mu    &   122.839   & 76.296    & 4.276 &  4.770    &  0.516      &   -0.3001     &  -0.2159    &  6.119 &  6.643    & 0.5006       &  4.160     & 3.778  & 4.301  & 4.781     & 0.507       \\
       & \sigma &   58.541     & 67.315    &   &     &        &      0.26164  &  0.2947   &   &     &        &   0.336    & 0.394   &    &    &        \\
       
GPT 3 \cite{brown2020language}  & \mu    &  122.839      &   72.495  & 4.276 & 2.906      &   0.505     &    -0.3001    & 0.0958    & 6.119 &  6.527     &  0.5041     &   4.160    &  3.620  & 4.301 & 2.913     &   0.486     \\
       & \sigma &      58.541  &  66.634   &    &    &        & 0.26164        &  0.3834   &  &      &        &   0.336 &  0.626  &  &      &        \\
Vicuna \cite{zhu2023minigpt}  & \mu    &   122.839     &  92.566   & 4.276  & 1.558     &   0.509     &  -0.3001      &  0.9088    &  6.119  & 0.801    &  0.5083      &   4.160    & 3.917   & 4.301 & 1.558      &     0.506   \\
       & \sigma &    58.541    &  66.077   &    &    &        &       0.26164 &  0.2927   &   &       &        &   0.336    &  0.639  &   &     &        \\
StableLM \cite{liu2023your}  & \mu    &   122.839     &  91.789   & 4.276   & 1.437    &  0.512       &  -0.3001      & 0.3507    & 6.119  & 6.323     &    0.5057    &   4.160    &  4.215  & 4.301 & 1.485      &  0.561      \\
       & \sigma &    58.541    &  66.629   &    &        &        &   0.26164 &  0.3717   &   &      &        &   0.336    & 0.618   &   &     &        \\

MPT \cite{MosaicML2023Introducing}  & \mu    &   122.839     &  76.105   & 4.276  & 1.446     &  0.512      &   -0.3001     &  0.3829   & 6.119  & 6.203      &   0.4969     &  4.160     &  3.774  & 4.301  & 1.501     &  0.501      \\
       & \sigma &    58.541    &  86.554   &      &  &        &       0.26164 &  0.4033   &   &     &        &    0.336   &  0.698  &   &     &        \\

LLaMA \cite{touvron2023llama}  & \mu    &  122.839      &  93.321   & 4.276  & 2.693     & 0.514       &    -0.3001    &  0.4578   & 6.119   & 4.435    &    0.496    &   4.160    & 3.979   & 4.301 &  2.705     &      0.504  \\
       & \sigma &   58.541     &  56.919   &  &      &        &      0.26164  &  0.5261   &   &     &        &   0.336    &  0.534  &   &     &        \\

Alpaca \cite{maeng2017alpaca}  & \mu    &   122.839     &  50.728   & 4.276 & 2.276      &    0.511    &   -0.3001     &  0.3122   &  6.119  & 6.563    &     0.5009   &    4.160   &  3.491  & 4.301 &  2.289     &    0.507    \\
       & \sigma &   58.541     &  50.740   &  &       &        &      0.26164  &   0.3066  & &       &        &    0.336   & 0.427   &   &     &        \\

GPT 2 \cite{radford2019language}  & \mu    &  143.198      & 39.897    & 3.423  & 1.195    &   0.505     & -0.2798      &  0.5509   & 6.144  & 5.923     &    0.5029    &   4.492    & 3.302   & 3.436 & 1.195      &    0.504    \\
       & \sigma &  60.866      &  42.341     &    &    &        &       0.2966 &   0.3587  &   &     &        &   0.332  &  0.514  & &       &        \\

Dolly \cite{wang2022self}  & \mu    &    122.839    &  75.358   & 4.276  & 3.199    &  0.497      &    -0.3001    &  0.0635    & 6.119  & 6.563    &     0.5017   &  4.160     & 3.842   & 4.301 & 3.206      &    0.502    \\
       & \sigma &   58.541     &  75.358   &  &      &        &       0.26164 &  0.2741   &  &        &        &   0.336    &  0.369  &  &       &        \\

BLOOM \cite{scao2022bloom}  & \mu    &   106.776     &  104.091   & 3.378  & 2.712     &  0.532      &  -0.2992      &  -0.0153
  & 6.138  &  6.563   &    0.4936    &   4.297    & 4.185  & 3.406  & 2.765     &     0.498   \\
       & \sigma &  57.091     & 62.152     &  &      &        &     0.2416   & 0.0032    &  &      &        & 0.338      &  0.535  &   &     &        \\
       

T0 \cite{sanh2021multitask}  & \mu    &    122.839    &  46.980   & 4.276  & 0.133     &   0.515     &  -0.3001      &  0.9171   & 6.119  & 0.880     &   0.5104     &    4.160   & 3.302   & 4.301  & 0.133   &    0.503    \\
       & \sigma &  58.541      &  79.224   &      &  &        &       0.26164 &  0.2420   &  &      &        &   0.336    & 0.765   &    &    &        \\
       
XLNet \cite{yang2019xlnet}  & \mu    &  50.073      & 35.465    &   4.222  &   1.118      &   0.492     &  -0.4010      & 0.3920    &  6.152 &    5.893    &   0.5004     &   2.123    & 1.966   &  4.254 &   1.138      &      0.503  \\
       & \sigma & 36.411    & 80.836    &    &      &        &       0.26164 &  0.4021   &    &     &        &   0.535    &  0.934  &     &   &        \\
T5 \cite{raffel2020exploring}  & \mu    &    122.839    &  43.495   & 4.276 &  0.777      &  0.519     &   -0.3001     &  0.6645   &  6.119 & 4.290     &    0.5052    &  4.160     &  3.175  & 4.301 & 0.805      &   0.505     \\
       & \sigma &   58.541     &  65.178   &   &      &        &       0.26164 &  0.3956   &  &       &        &   0.336    & 0.754   &  &       &        \\
       \bottomrule
\end{tabular}%
}
\caption{Comprehensive table for all 15 LLMs with statistical measures for Perplexity, Burstiness, and NLC, along with bootstrap p values ($\alpha$ = 0.05), indicating non-significance for b-values greater than the chosen alpha level.}
\label{tab:perp-burst-nlc-compile-full}
\end{table*}   
\end{comment}


\begin{comment}
\section{Entropy}
The concept of entropy is also used to measure the degree of uncertainty and randomness in language models and texts. When the probability distribution is distributed among the words or tokens more evenly, the entropy of a language model or text is higher, indicating that the text contains a larger level of uncertainty or unpredictability. The probability distribution of words in a language model is used to determine perplexity, which can be seen as the exponentiated entropy. In comparison to a model with a higher perplexity, one with a lower perplexity performs better at word prediction. Thus, producing text that is fluent and coherent requires a language model with a lower perplexity. When the probability distribution of words in a language model is more evenly spread out, the entropy is higher and the perplexity is lower. As a result, a language model with a larger entropy will likely be less perplexing because it is more unpredictable. 

\textcolor{orange}{Hence, we have also experimented with all 15 models using entropy as a measure to detect statistical significance between entropies of human-written vs AI-generated text. Table \ref{tab:perp-burst-nlc-compile} showcases our findings.}

\begin{comment}
\begin{table}[htp]
\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}clcc@{}}
\toprule
\multicolumn{2}{c}{\textbf{Models}} & \textbf{AI Text} & \textbf{Human Text} \\
\midrule
\multirow{2}{*}{\textbf{OPT}}  & \textbf{$\mu$}  & 3.764  & 4.209   \\
    % & \textbf{variance}       & 0.357  & 0.492 \\
    & \textbf{$\sigma$} & 0.128   & 0.242  \\ 
    \cmidrule(l){3-4} 
\multirow{2}{*}{\textbf{XLNet}} & \textbf{$\mu$}  & 2.362  & 2.528   \\
    % & \textbf{variance}       & 0.505  & 0.904  \\
    & \textbf{$\sigma$} & 0.255 & 0.817  \\ 
\toprule
\end{tabular}%
}
\caption{Statistical measures of Entropy in AI vs Human Text for Models OPT and XLNet}
\label{table:opt-xlnet-stat}
\end{table}
\end{comment}


\begin{longtblr}[
  caption = {AI generated text for a sample prompt given to all 15 LLMs},
  label = {tab:example1},
]{
  colspec = {|X|X[4]|},
  rowhead = 1
} 
\textbf{{\footnotesize hist}}  &  \textit{{\footnotesize line}} \\
\includegraphics[width=\textwidth]{perp_plots/gpt4-HP.pdf}  &     \includegraphics[width=\textwidth]{perp_plots/gpt4-HP.pdf}\\
\end{longtblr}


\begin{figure*}[!htbp]
\centering
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt4-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt4-LP.pdf}
\end{minipage}%
\subcaption{GPT4}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt3-5-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt3-5-LP.pdf}
\end{minipage}%
\subcaption{GPT3.5}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/opt-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/OPT-LP.pdf}
\end{minipage}%
\subcaption{OPT}
\label{fig:hist-line-perp-plot}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt3-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt3-LP.pdf}
\end{minipage}%
\subcaption{GPT3}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/vicuna-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/vicuna-LP.pdf}
\end{minipage}%
\subcaption{Vicuna}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/stablelm-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/stablelm-LP.pdf}
\end{minipage}%
\subcaption{StableLM}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/mpt-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/mpt-LP.pdf}
\end{minipage}%
\subcaption{MPT}
\label{fig:hist-line-perp-plot}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/llama-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/llama-LP.pdf}
\end{minipage}%
\subcaption{LLaMA}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/alpaca-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/alpaca-LP.pdf}
\end{minipage}%
\subcaption{Alpaca}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt2-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/gpt2-LP.pdf}
\end{minipage}%
\subcaption{GPT2}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/dolly-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/dolly-LP.pdf}
\end{minipage}%
\subcaption{Dolly}
\label{fig:hist-line-perp-plot}
\end{figure*}

\begin{figure*}[!htbp]
\centering
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/bloom-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/bloom-LP.pdf}
\end{minipage}%
\subcaption{BLOOM}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t0-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t0-LP.pdf}
\end{minipage}%
\subcaption{T0}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/xlnet-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/xlnet-LP.pdf}
\end{minipage}%
\subcaption{XLNet}
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t5-HP.pdf}
\end{minipage}%
\begin{minipage}{.45\textwidth}
  \centering
\includegraphics[width=\textwidth]{perp_plots/t5-LP.pdf}
\end{minipage}%
\subcaption{T5}
\label{fig:hist-line-perp-plot}
\end{figure*}

